Wan-Weaver: Interleaved Multi-modal Generation via Decoupled Training

Recent unified models have made unprecedented progress in both understanding and generation. However, while most of them accept multi-modal inputs, they typically produce only single-modality outputs. This challenge of producing interleaved content is mainly due to training data scarcity and the difficulty of modeling long-range cross-modal context. To address this issue, we decompose interleaved generation into textual planning and visual consistency modeling, and introduce a framework consisting of a planner and a visualizer. The planner produces dense textual descriptions for visual content, while the visualizer synthesizes images accordingly. Under this guidance, we construct large-scale textual-proxy interleaved data (where visual content is represented in text) to train the planner, and curate reference-guided image data to train the visualizer. These designs give rise to Wan-Weaver, which exhibits emergent interleaved generation ability with long-range textual coherence and visual consistency. Meanwhile, the integration of diverse understanding and generation data into planner training enables Wan-Weaver to achieve robust task reasoning and generation proficiency. To assess the model's capability in interleaved generation, we further construct a benchmark that spans a wide range of use cases across multiple dimensions. Extensive experiments demonstrate that, even without access to any real interleaved data, Wan-Weaver achieves superior performance over existing methods.

==> tables/weaver_bench.tex <==
\begin{table}[!t]
    \caption{Quantitative comparison on WeaverBench. PA: Prompt Adherence, NC: Narrative Coordination, CC: Content Consistency, IC: Image Consistency, CP: Completeness.}
    \label{tab:weaver_bench_results}
    \vspace{-0.5em}


    \resizebox{\linewidth}{!}{
    % \setlength{\tabcolsep}{2.1pt}
    \centering
    \begin{tabular}{lccccc|c}
        \toprule
        % \rowcolor{headerblue}
        Method  & PA & NC & CC & IC & CP & Overall \\
        \midrule
        Orthus & 2.47& 1.88& 1.69& 1.51& 1.91& 1.89\\
        Anole & 4.14& 3.76&  3.77& 3.42& 3.64&3.74 \\
        Emu3.5 & 7.65& 7.55&  7.56& 7.50& 7.41& 7.53\\
        Nano Banana & \seco{8.53}& \seco{8.19}& \best{8.53}& \best{8.38}& \seco{8.29}&\seco{8.38}\\
        \rowcolor{Gray}
        Wan-Weaver (Ours) &\best{8.71} &\best{8.33} &\seco{8.50} &\seco{8.13} &\best{8.46} &\best{8.43}\\
        \bottomrule
    \end{tabular}
    
}
\vspace{-1em}
\end{table}
